Proofs of No Intrusion

A central challenge in data security is not just preventing theft, but detecting whether it has occurred. Classically, this is impossible because a perfect copy leaves no evidence. Quantum mechanics, on the other hand, forbids general duplication, opening up new possibilities. We introduce Proofs of No Intrusion, which enable a classical client to remotely test whether a quantum server has been hacked and the client's data stolen. Crucially, the test does not destroy the data being tested, avoiding the need to store a backup elsewhere. We define and construct proofs of no intrusion for ciphertexts assuming fully homomorphic encryption. Additionally, we show how to equip several constructions of unclonable primitives with proofs of non-intrusion, such as unclonable decryption keys and signature tokens. Conceptually, proofs of non-intrusion can be defined for essentially any unclonable primitive. At the heart of our techniques is a new method for non-destructively testing coset states with classical communication. It can be viewed as a non-destructive proof of knowledge of a measurement result of the coset state.

==> general_macros.tex <==
\RequirePackage[colorinlistoftodos]{todonotes}
\newcommand{\authnote}[4]{\todo[inline,caption={},bordercolor=#3,linecolor=#2,color=#2]{\footnotesize{\sc \bf #1:} #4}{}}
\newcommand{\justin}[1]{\ifnotes\authnote{Justin}{lime}{green!25!brown}{#1}\fi}
\definecolor{cyan}{rgb}{0,255,255}
\newcommand{\vipul}[1]{\ifnotes\authnote{Vipul}{cyan}{blue}{#1}\fi}

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}


\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}


%%%%%%%%%%%% Quantum %%%%%%%%%%%%%%%%
\newcommand{\ketbra}[1]{\ket{#1}\bra{#1}}
\newcommand{\Tr}{\mathsf{Tr}}
\newcommand{\trace}{\Tr}

\newcommand{\regA}{\mathcal{A}}
\newcommand{\regB}{\mathcal{B}}
\newcommand{\regC}{\mathcal{C}}
\newcommand{\regD}{\mathcal{D}}
\newcommand{\regE}{\mathcal{E}}
\newcommand{\regF}{\mathcal{F}}
\newcommand{\regG}{\mathcal{G}}
\newcommand{\regH}{\mathcal{H}}
\newcommand{\regI}{\mathcal{I}}
\newcommand{\regJ}{\mathcal{J}}
\newcommand{\regK}{\mathcal{K}}
\newcommand{\regL}{\mathcal{L}}
\newcommand{\regM}{\mathcal{M}}
\newcommand{\regN}{\mathcal{N}}
\newcommand{\regO}{\mathcal{O}}
\newcommand{\regP}{\mathcal{P}}
\newcommand{\regQ}{\mathcal{Q}}
\newcommand{\regR}{\mathcal{R}}
\newcommand{\regS}{\mathcal{S}}
\newcommand{\regT}{\mathcal{T}}
\newcommand{\regU}{\mathcal{U}}
\newcommand{\regV}{\mathcal{V}}
\newcommand{\regW}{\mathcal{W}}
\newcommand{\regX}{\mathcal{X}}
\newcommand{\regY}{\mathcal{Y}}
\newcommand{\regZ}{\mathcal{Z}}

%%%%%%%%%%% Misc %%%%%%%%%%

\newcommand{\intersect}{\cap}
\newcommand{\Span}{\mathsf{Span}}
\newcommand{\diff}[1]{{\color{red}#1}}

%%%%%%%%%%%% Theorem-Like Environments %%%%%%%%%%

\ifsubmission
\else
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{subclaim}{Sub-Claim}
\newtheorem{fact}{Fact}
\newtheorem{property}{Property}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\theoremstyle{definition}
\fi
\newtheorem{construction}{Construction}

%%%%%%%%%%%%%%%%%% Crypto %%%%%%%%%%%%%%%
\newcommand{\KeyGen}{\mathsf{KeyGen}}
\newcommand{\Enc}{\mathsf{Enc}}
\newcommand{\Dec}{\mathsf{Dec}}
\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\MAC}{\mathsf{MAC}}
\newcommand{\Sign}{\mathsf{Sign}}
\newcommand{\Ver}{\mathsf{Ver}}
